A Kernel Based High Order "Explicit" Unconditionally Stable Constrained Transport Method for Ideal Magnetohydrodynamics

The ideal Magnetohydrodynamics (MHD) equations are challenging because one needs to maintain the divergence free condition, $\nabla \cdot \Bv = 0$. Many numerical methods have been developed to enforce this condition. In this work, we further our work on mesh aligned constrained transport by developing a new kernel based approach for the vector potential in 2D and 3D. The approach for solving the vector potential is based on the method of lines transpose and is A-stable, eliminating the need for diffusion limiters needed in our previous work in 3D. The work presented here is an improvement over the previous method in the context of problems with strong shocks due to the fact that we could eliminate the diffusion limiter that was needed in our previous version of constrained transport. The method is robust and has been tested on the 2D and 3D cloud shock, blast wave and field loop problems.

==> demo_citation.tex <==
\section{Demo Citation}

**************************************************************************************
\par Demo Citations for Reference papers in Yan's paper.

\par Reference paper in Yan's paper:  \cite{jia2008krylov}. 
 Reference paper in Yan's paper:  \cite{kropinski2011fast}. 
 Reference paper in Yan's paper:  \cite{ketcheson2011step}. 
 Reference paper in Yan's paper:  \cite{liu2011high}. 
 Reference paper in Yan's paper:  \cite{hajipour2012high}. 
 Reference paper in Yan's paper:  \cite{zhang2009numerical}. 
 Reference paper in Yan's paper:  \cite{aregba2004explicit}. 
 Reference paper in Yan's paper:  \cite{cavalli2007high}. 
 Reference paper in Yan's paper:  \cite{bessemoulin2012finite}. 
 Reference paper in Yan's paper:  \cite{abedian2013high}. 
 Reference paper in Yan's paper:  \cite{shu2002survey}. 
 Reference paper in Yan's paper:  \cite{gottlieb2001strong}. 
 Reference paper in Yan's paper:  \cite{gottlieb2005high}. 
 Reference paper in Yan's paper:  \cite{schemann1998adaptive}. 
 Reference paper in Yan's paper:  \cite{causley2014method}. 
 Reference paper in Yan's paper:  \cite{causley2014higher}. 
 Reference paper in Yan's paper:  \cite{causley2013method}. 
 Reference paper in Yan's paper:  \cite{causley2016method}. 
 Reference paper in Yan's paper:  \cite{causley2017method}. 
 Reference paper in Yan's paper:  \cite{cheng2017asymptotic}. 
 Reference paper in Yan's paper:  \cite{christlieb2016weno}. 
 Reference paper in Yan's paper:  \cite{muskat1937flow}. There is no journal for this citation!!
 Reference paper in Yan's paper:  \cite{aronson1986porous}. 
 Reference paper in Yan's paper:  \cite{zel1950towards}. 
 Reference paper in Yan's paper:  \cite{barenblatt1952self}. 
 Reference paper in Yan's paper:  \cite{alt1983quasilinear}. 
 Reference paper in Yan's paper:  \cite{duyn1982nonstationary}. 
 Reference paper in Yan's paper:  \cite{otto1996l1}. 
 Reference paper in Yan's paper:  \cite{buckley1942mechanism}. 
 Reference paper in Yan's paper:  \cite{kurganov2000new}. 
 Reference paper in Yan's paper:  \cite{liu1994weighted}. 
 Reference paper in Yan's paper:  \cite{jiang1996efficient}. 
 Reference paper in Yan's paper:  \cite{balsara2000monotonicity}. 
 Reference paper in Yan's paper:  \cite{shu2009high}. 
 Reference paper in Yan's paper:  \cite{shu1998essentially}. 
 Reference paper in Yan's paper:  \cite{chou2006high}. 
 Reference paper in Yan's paper:  \cite{chou2007high}. 
 Reference paper in Yan's paper:  \cite{liu2009positivity}. 
 Reference paper in Yan's paper:  \cite{borges2008improved}. 
 Reference paper in Yan's paper:  \cite{ascher1997implicit}. 
 Reference paper in Yan's paper:  \cite{Hairer1996}. 
 Reference paper in Yan's paper:  \cite{greengard1987fast}. 
 Reference paper in Yan's paper:  \cite{barnes1986hierarchical}. 
 Reference paper in Yan's paper:  \cite{christlieb2017kernel}. 
 Reference paper in Yan's paper:  \cite{huang2008numerical}. 
 Reference paper in Yan's paper:  \cite{xiong2010fast}. 
 Reference paper in Yan's paper:  \cite{zhang2011uniformly}. 
 Reference paper in Yan's paper:  \cite{crandall1983viscosity}. 
 Reference paper in Yan's paper:  \cite{crandall1984some}. 
 Reference paper in Yan's paper:  \cite{osher1988fronts}. 
 Reference paper in Yan's paper:  \cite{osher1991high}. 
 Reference paper in Yan's paper:  \cite{jiang2000weighted}. 
 Reference paper in Yan's paper:  \cite{zhang2003high}. 
 Reference paper in Yan's paper:  \cite{shu2007high}. 
 Reference paper in Yan's paper:  \cite{hu1999discontinuous}. 
 Reference paper in Yan's paper:  \cite{lepsky2000analysis}. 
 Reference paper in Yan's paper:  \cite{cheng2007discontinuous}. 
 Reference paper in Yan's paper:  \cite{cheng2014new}. 
 Reference paper in Yan's paper:  \cite{yan2011local}. 
 Reference paper in Yan's paper:  \cite{qiu2005hermite}. 
 Reference paper in Yan's paper:  \cite{qiu2007hermite}. 
 Reference paper in Yan's paper:  \cite{tao2017dimension}. 
 Reference paper in Yan's paper:  \cite{zheng2017finite}. 
 Reference paper in Yan's paper:  \cite{crandall1984two}. 
 Reference paper in Yan's paper:  \cite{abgrall1996numerical}. 
 Reference paper in Yan's paper:  \cite{lafon1996high}. 
 Reference paper in Yan's paper:  \cite{zhu2013hermite}. 
 Reference paper in Yan's paper:  \cite{tan2010inverse}. 
 Reference paper in Yan's paper:  \cite{tan2012efficient}. 
 Reference paper in Yan's paper:  \cite{darbon2016algorithms}. 
 Reference paper in Yan's paper:  \cite{chow2017algorithm}. 


\par ******************************************************************************
\par Demo Citations for Reference paper in Qi's paper

\par Reference paper in Qi's paper:  \cite{balsara2001divergence}. 
 Reference paper in Qi's paper:  \cite{balsara2004second}. 
 Reference paper in Qi's paper:  \cite{balsara2009divergence}. 
 Reference paper in Qi's paper:  \cite{balsara2012self}.
 Reference paper in Qi's paper:  \cite{balsara2004comparison}. 
 Reference paper in Qi's paper:  \cite{balsara2013efficient}.
 Reference paper in Qi's paper:  \cite{balsara2009efficient}. 
 Reference paper in Qi's paper:  \cite{balsara1999staggered}. 
 Reference paper in Qi's paper:  \cite{barth1999numerical}.
  Reference paper in Qi's paper:  \cite{brio1988upwind}. 
 Reference paper in Qi's paper:  \cite{cargo1997roe}.
  Reference paper in Qi's paper:  \cite{cheng2013positivity}.
  Reference paper in Qi's paper:  \cite{dafermos2005hyperbolic}.
  Reference paper in Qi's paper:  \cite{dai1998simple}.
  Reference paper in Qi's paper:  \cite{dedner2002hyperbolic}.
  Reference paper in Qi's paper:  \cite{devore1991flux}.
  Reference paper in Qi's paper:  \cite{evans1988simulation}. 
 Reference paper in Qi's paper:  \cite{fey2003constrained}. 
 Reference paper in Qi's paper:  \cite{gottlieb2009high}.
  Reference paper in Qi's paper:  \cite{helzel2011unstaggered}.
  Reference paper in Qi's paper:  \cite{helzel2013high}.
% \par Reference paper in Qi's paper:  \cite{jiang2000weighted}. common paper ref with Yan!!!
  Reference paper in Qi's paper:  \cite{jiang1996efficient}.
  Reference paper in Qi's paper:  \cite{jiang1999high}.
  Reference paper in Qi's paper:  \cite{kawai2013divergence}.
  Reference paper in Qi's paper:  \cite{ketcheson2008highly}.
  Reference paper in Qi's paper:  \cite{leveque1997wave}.
  Reference paper in Qi's paper:  \cite{li2005locally}.
  Reference paper in Qi's paper:  \cite{li2011central}.
  Reference paper in Qi's paper:  \cite{londrillo2000high}.
  Reference paper in Qi's paper:  \cite{londrillo2004divergence}.
 Reference paper in Qi's paper:  \cite{parks1991physics}. make sure if this is the correct ref.Qi de 2004 demis
  Reference paper in Qi's paper:  \cite{powell1994approximate}.
  Reference paper in Qi's paper:  \cite{powell1999solution}.
 Reference paper in Qi's paper:  \cite{rossmanith2006unstaggered}.
  Reference paper in Qi's paper:  \cite{ryu1998divergence}.
  Reference paper in Qi's paper:  \cite{seal2014high}. 
 Reference paper in Qi's paper:  \cite{shen2011adaptive}. 
 Reference paper in Qi's paper:  \cite{shu1998essentially}.
  Reference paper in Qi's paper:  \cite{shu2009high}.
  Reference paper in Qi's paper:  \cite{de2001multi}.
  Reference paper in Qi's paper:  \cite{torrilhon2005locally}.
  Reference paper in Qi's paper:  \cite{toth2000b}. 
 Reference paper in Qi's paper:  \cite{yee1966numerical}.
  Reference paper in Qi's paper:  \cite{zachary1994higher}.
  Reference paper in Qi's paper:  \cite{zhang2011maximum}. 

\par Reference paper in Qi's paper:  \cite{mhDclaw}. 

\par ******************************************************************************
\par SONRADAN EKLENEN MAKALELER
1. Qi'nin makalesi  \cite{christlieb2014finite}
2. Yan'in molt-HJ \cite{christlieb2019kernel}






